Pronoun-Targeted Fine-tuning for NMT with Hybrid Losses

Popular Neural Machine Translation model training uses strategies like backtranslation to improve BLEU scores, requiring large amounts of additional data and training. We introduce a class of conditional generative-discriminative hybrid losses that we use to fine-tune a trained machine translation model. Through a combination of targeted fine-tuning objectives and intuitive re-use of the training data the model has failed to adequately learn from, we improve the model performance of both a sentence-level and a contextual model without using any additional data. We target the improvement of pronoun translations through our fine-tuning and evaluate our models on a pronoun benchmark testset. Our sentence-level model shows a 0.5 BLEU improvement on both the WMT14 and the IWSLT13 De-En testsets, while our contextual model achieves the best results, improving from 31.81 to 32 BLEU on WMT14 De-En testset, and from 32.10 to 33.13 on the IWSLT13 De-En testset, with corresponding improvements in pronoun translation. We further show the generalizability of our method by reproducing the improvements on two additional language pairs, Fr-En and Cs-En. Code available at <https://github.com/ntunlp/pronoun-finetuning>.

==> results.tex <==
\begin{table*}[bh]
%\begin{figure}[h]
%\caption{Image paragraph captioning experimental results and human evaluation for auto-completion.}
%\label{table:img-para_all}
%\begin{minipage}[t]{0.49\textwidth}
\begin{subtable}[t]{0.5\textwidth}
    \centering
     \scalebox{0.7}{\begin{tabular}{lccccc}
\toprule
 & \textbf{WMT14}  & \multicolumn{4}{c}{\textbf{Pronoun Testset}} \\
\textbf{Model} & \textbf{BLEU} & \textbf{BLEU}  &\textbf{P} & \textbf{R} &\textbf{F1} \\ 
\midrule
\multicolumn{6}{c}{\textbf{All tokens}} \\
\midrule
%\textbf{\sts} & & & & \\
 \sts & \textbf{32.14} & 36.16 & 78.83 & 66.15 & 69.77 \\
 \rand & 31.86 & 35.88 & 78.07 & 66.00 & 69.65 \\
 \full & 31.75 & 36.34 & 78.27 & 66.36 & 69.91 \\
 \concat & 31.75 & \textbf{36.70} & \textbf{81.25} & \textbf{69.27} & \textbf{72.88} \\
 %$D_{rand}$ & 31.86 & - & - & - \\

 \midrule
 
 \multicolumn{6}{c}{\textbf{Only Pronouns}} \\
 \midrule

 \sts & 31.81 & 36.43 & 78.62 & 66.82 & 70.37 \\
 \rand & 31.71 & 36.12 & 78.65 & 66.72 & 70.32 \\
 \full & 31.89 & 36.20 &  78.31 & 66.32 & 69.98 \\
 \concat & \textbf{31.99} & \textbf{36.64} & \textbf{80.87} & \textbf{69.07} & \textbf{72.64} \\

\bottomrule
\end{tabular}}
\label{table:pairwise_loss_results}
\end{subtable}
%\end{minipage}
\hfill
\begin{subtable}[t]{0.5\textwidth}
%\begin{minipage}[t]{0.49\textwidth}
\centering
     \scalebox{0.7}{\begin{tabular}{lccccc}
\toprule
 & \textbf{WMT14}  & \multicolumn{4}{c}{\textbf{Pronoun Testset}} \\
\textbf{Model} & \textbf{BLEU} & \textbf{BLEU}  &\textbf{P} & \textbf{R} &\textbf{F1} \\ 
\midrule
\multicolumn{6}{c}{\textbf{All tokens}} \\
\midrule 
%\textbf{\sts} & & & & \\
 \sts & 31.83 & 36.50 & 79.18 & 67.16 & 70.78 \\
 \rand & 31.73 & 36.16 & 78.32 & 66.62 & 70.15 \\
 \full & 31.77 & 36.24 &  78.35 & 66.17 & 69.86 \\
 \concat & \textbf{31.85} & \textbf{36.61}  & \textbf{80.91} & \textbf{68.91} & \textbf{72.57} \\
 %$D_{rand}$ & 31.86 & - & - & - \\

 \midrule
 
 \multicolumn{6}{c}{\textbf{Only Pronouns}} \\
 \midrule

 \sts & 31.73 & 36.30 & 79.01 & 66.80 & 70.50 \\
 \rand  & \textbf{32.05} & 36.43  & 78.35 & 66.25 & 69.87 \\
 \full & \textbf{32.05} & 35.81 & 78.58 & 66.52 & 70.22 \\
 \concat & \textbf{32.00} & \textbf{36.57} & \textbf{80.89} & \textbf{68.66} & \textbf{72.39} \\
\bottomrule
\end{tabular}}
\label{table:nll_loss_results}
\end{subtable}
%\end{minipage}
% \hfill
% \begin{minipage}[t]{0.48\textwidth}
%     \centering
%     \captionof{table}{Results for image paragraph captioning.}
%     % on the Visual Genome testset.}
%     \label{table:resultsimg-para}
%     \scalebox{0.95}{\begin{tabular}{lc}
%     \toprule
%     \bf{Models} &  \bf{CIDEr}  \\
%     \midrule
%     \text{MLE} w/o 3-block & {10.51}\\
%     UL w/o 3-block ($\alpha$=0.5)  \quad \quad \quad& 14.65 \\
%     \textsc{SG} w/o 3-block ($\gamma$=0.5) & \bf{19.42} \\
%     \midrule
%     \text{MLE} w/ 3-block & 22.77\\
%     UL w/ 3-block ($\alpha$=0.5) & {22.25} \\
%     \textsc{SG} w/ 3-block ($\gamma$=0.5) & \bf{24.62} \\
%     \bottomrule
%   \end{tabular}}
% \end{minipage}
 \captionof{table}{Additional finetuning loss: finetuning results on the WMT14 De-En testset with F1 scores on the pronoun testset. Results reported for \sts\ and \concat\ are based on alternated training with pronoun-targeted finetuning data $\gD^{'}$ and the upsampled full training data ($2 * \gD$). Results reported for \rand\ are based on alternated training with a random subset and the upsampled full data ($2 * \gD$), and results reported for \full\ are based on additional training with the full training dataset $\gD$.}
%     % \textbf{AC1} agreements for the ranking of generated texts between humans. }
 \label{table:add_loss_results}
\vspace{-1em}
\end{table*}


% \begin{table}[t]
% \centering
% \scalebox{0.80}{\begin{tabular}{lccccc}
% \toprule
%  & \textbf{WMT14}  & \multicolumn{4}{c}{\textbf{Pronoun Testset}} \\
% \textbf{Model} & \textbf{BLEU} & \textbf{BLEU}  &\textbf{P} & \textbf{R} &\textbf{F1} \\ 
% \midrule
% \multicolumn{6}{c}{\textbf{All tokens}} \\
% \midrule 
% %\textbf{\sts} & & & & \\
%  \sts & 31.83 & 36.50 & 79.18 & 67.16 & 70.78 \\
%  \rand & 31.73 & 36.16 & 78.32 & 66.62 & 70.15 \\
%  \full & 31.77 & 36.24 &  78.35 & 66.17 & 69.86 \\
%  \concat & \textbf{31.85} & \textbf{36.61}  & \textbf{80.91} & \textbf{68.91} & \textbf{72.57} \\
%  %$D_{rand}$ & 31.86 & - & - & - \\

%  \midrule
 
%  \multicolumn{6}{c}{\textbf{Only Pronouns}} \\
%  \midrule

%  \sts & 31.73 & 36.30 & 79.01 & 66.80 & 70.50 \\
%  \rand  & \textbf{32.05} & 36.43  & 78.35 & 66.25 & 69.87 \\
%  \full & \textbf{32.05} & 35.81 & 78.58 & 66.52 & 70.22 \\
%  \concat & \textbf{32.00} & \textbf{36.57} & \textbf{80.89} & \textbf{68.66} & \textbf{72.39} \\


 
% \bottomrule
% \end{tabular}}

% \caption{Additional log-likelihood loss: finetuning results on the WMT14 De-En testset with F1 scores on the pronoun testset. Results reported for \sts\ and \concat\ are based on alternated training with pronoun-targeted finetuning data and the upsampled primary training data. Results reported for \rand\ are based on alternated training with a random subset and the upsampled primary data, and results reported for \full\ are based on additional training with the full training dataset. }
% \label{table:nll_loss_results}

% \end{table}
